Latitude-dependent Atmospheric Waves and Long-period Modulations in Luhman 16 B from the Longest Lightcurve of an Extrasolar World

In this work, we present the longest photometric monitoring of up to 1200 hours of the strongly variable brown-dwarf binaries Luhman 16 AB and provide evidence of $\pm$5% variability on a timescale of several-to-hundreds of hours for this object. We show that short-period rotational modulation around 5 hours (k = 1 wavenumber) and 2.5 hours (k = 2 wavenumber) dominate the variability under 10 hours, where the planetary-scale waves model composed of k = 1 and k = 2 waves provides good fits to both the periodogram and light curve. In particular, models consisting of three to four sine waves could explain the variability of light curve durations up to 100 hours. We show that the relative range of k = 2 periods is narrower compared to k = 1 period. Using simple models of zonal banding in Solar System giants, we suggest that the difference in period range arises from the difference in windspeed distribution at low and mid-to-high latitudes in the atmosphere. Lastly, we show that Luhman 16 AB also exhibits long-period $\pm$5% variability with periods ranging from 15 hours up to 100 hours over the longest monitoring of this object. Our results on k = 1 and k = 2 waves and long-period evolution are consistent with previous 3D atmosphere simulations, demonstrating that both latitude-dependent waves and slow-varying atmospheric features are potentially present in Luhman 16 AB atmospheres and are significant contribution to the light curve modulation over hundreds of rotations.

==> author_affiliations.tex <==
\author[0000-0003-3714-5855]{Dániel Apai}
\affil{Steward Observatory, The University of Arizona, 933 N. Cherry Avenue, Tucson, AZ 85721, USA}
\affiliation{Lunar and Planetary Laboratory, University of Arizona, 1640 E. University Boulevard, Tucson, AZ 85721, USA}

\author[0000-0003-1149-3659]{Domenico Nardiello}
\affil{INAF—Osservatorio Astronomico di Padova, Vicolo dell’Osservatorio 5, I-35122, Padova, Italy}

\author[0000-0003-4080-6466]{Luigi R. Bedin}
\affil{INAF—Osservatorio Astronomico di Padova, Vicolo dell’Osservatorio 5, I-35122, Padova, Italy}

\author[0000-0001-7356-6652]{Theodora Karalidi}
\affil{Department of Physics, University of Central Florida, 4111 Libra Dr, Orlando, FL 32816, USA}

\author[0000-0003-2278-6932]{Xianyu Tan}
\affil{Tsung-Dao Lee Institute, Shanghai Jiao Tong University, 520 Shengrong Road, Shanghai, People’s Republic of China}
\affil{School of Physics and Astronomy, Shanghai Jiao Tong University, 800 Dongchuan Road, Shanghai, People’s Republic of China}
